Liquid interfaces in viscous straining flows: Numerical studies of the selective withdrawal transition

This paper presents a numerical analysis of the transition from selective withdrawal to viscous entrainment. In our model problem, an interface between two immiscible layers of equal viscosity is deformed by an axisymmetric withdrawal flow, which is driven by a point sink located some distance above the interface in the upper layer. We find that steady-state hump solutions, corresponding to selective withdrawal of liquid from the upper layer, cease to exist above a threshold withdrawal flux, and that this transition corresponds to a saddle-node bifurcation for the hump solutions. Numerical results on the shape evolution of the steady-state interface are compared against previous experimental measurements. We find good agreement where the data overlap. However, the numerical results' larger dynamic range allows us to show that the large increase in the curvature of the hump tip near transition is not consistent with an approach towards a power-law cusp shape, an interpretation previously suggested from inspection of the experimental measurements alone. Instead the large increase in the curvature at the hump tip reflects a logarithmic coupling between the overall height of the hump and the curvature at the tip of the hump.

==> background_bkup.tex <==
%auto-ignore
%% July 27 2006
%\section{Background}
Many different realizations of flow-driven topological transitions
have been investigated in previous works. Here, we review 
those studies that directly relate to the ingredients necessary for a 
topological transition to take place and the role of singularities 
and saddle node bifurcations in the interface evolution. 

%In other words, does
%the steady-state shape approach a singular shape as the transition is
%approached? If it does, is it possible to attain the singular solution
%by tuning material parameters and/or boundary conditions in the problem? 
{\it Viscous entrainment in the absence of surface tension}\\
A number of experimental and theoretical works have focused on
the transition from selective withdrawal to viscous entrainment in
stratified, two-layer systems where surface tension effects are assumed
to be either negligible or weak. These studies were motivated by
geophysical flows, in particular the emptying of a magma chamber 
during a volcanic explosion. Blake \& Ivey investigated the threshold
withdrawal flux $\tilde{Q}_c$ necessary for the onset of entrainment
in miscible, stratified layers~(\cite{ivey85}). In a follow up numerical 
study~(\cite{Lister89}), Lister analyzed the onset of entrainment in two 
liquid layers of equal 
viscosity and found that a finite value for $\tilde{Q}_c$ exists only 
if surface tension effects, however small, are included in the analysis.  
Further annalysis of the hump evolution near the transition was not 
addressed in these studies.

{\it 2-D analogues}\\
There are a number of 2-D flow-driven topological transitions which
resemble the selective withdrawal to viscous entrainment in some
aspects but also differ from it in important ways. Air entrainment,
such as occcurs in high-speed coating~(\cite{simpkins00}) and in the
impact of a jet of viscous liquid into a layer of the same viscous
liquid~(\cite{Lorenceau04}) is often accompanied by the interface
approaching a two-dimensional power-law cusp
shape~(\cite{Joseph91}). Jeong \& Moffatt showed analytically that, in
the idealized limit where air flow effects are negligible, there is no
transition from selective withdrawal to air
entrainment~(\cite{JeongMoffatt91}). Instead the interface shape
approaches a steady-state singularity in the shape of a power-law cusp
as the flow rate is increased towards infinity.  More recent thereotical
and experimental analyses~(\cite{Eggers01,lorenceau03}) showed that,
when air flow effects are included, they perturb the idealized
dynamics so that a transition to air entrainment occurs at finite flow
rate and the approach towards a steady-state singularity is cut-off at
a small lengthscale. Since the cut-off for air entrainment originates
from viscous stresses associated with air flow, the cut-off
lengthscale has a strong dependence on the viscosity contrast and
increases as $(\mu_0/\mu)^{4/3}$, where $\mu_0$ is the air
viscosity.  

{\it Selective withdrawal in 3D with surface tension}\\
In their studies of 3-D axisymetric selective withdrawal Cohen \& Nagel~(\cite{CohenNagel02})
used two liquids of comparable viscosities and measured
$\tilde{h}$, the hump height, and $\tilde{\kappa}$, the mean curvature at
the hump tip, as a function of the withdrawal flux $\tilde{Q}$. In a follow up 
study Cohen~(\cite{Cohen04}) analyzed the transition for different pairs of
liquids. In particular, the viscosity ratio, defined as the viscosity
of the liquid to be entrained divided by the viscosity of the
entraining liquid, was varied from $O(1)$ to $10^{-3}$. 
Analysis of the measurements show that, as the transition from
selective withdrawal to viscous entrainment is approached from below,
the steady state hump curvature increases dramatically. Cohen and Nagel 
showed that this rate of increase can be fit to a power law divergence. 
They also noted however, that the hump never reaches a cusp shape. Instead 
the final stage of the hump evolution is cut off by the transition. This 
behavior lead to the interpretation that a singular solution organizes the 
nearly continuous transition between the steady-state hump and spout shapes. 
The transition from a hump to a spout was observed to occur when the radius 
of curvature at the hump tip was O($50$) $\mu$m or more. Moreover, the transition 
cut-off showed little dependence on the viscosity contrast between the two 
layers. Consequently axisymmetric viscous withdrawal in 3D differes strikingly 
from viscous withdrawal in 2D which shows a strong cut-off dependence 
on the viscosity contrast. 

{\it Viscous drainage}\\
An analogous, but not equivalent, topology change occurs in viscous
drainage experiments, in which a viscous liquid exposed to air is
placed in a container with an open aperture at the bottom surface and is
allowed to drain out of the container due to its own
weight~(\cite{Chaieb_preprint,sylvain06}).  The drainage creates a
large-scale toroidal recirculation whose viscous stresses deform the
interface, as occurs in the experiments by Cohen \& Nagel. Thus the
drainage experiment resemble an upside-down version of 
the two-layer withdrawl experiment. A key difference between
the two realizations is that the layer depth of the withdrawn fluid 
changes with time in the drainage experiment, but remains constant in the setup used by Cohen
\& Nagel.  As the liquid drains out and the layer depth decreases below a
critical value, a sharp cusp develops on the interface, a feature
identified by Correch du Pont \& Eggers as a steady-state singularity.  
A further decrease in the layer depth causes the cusp to
approach closer to the bottom surface and eventually intrude into the
aperture through which the fluid is draining. Correch du Pont \& Eggers 
report that there is no transition from selective withdrawal to viscous 
entrainment throughout the entire drainage process. Moreover,
the maximum curvature obtained in the drainage experiments, which
corresponds to using two fluid layers with a viscosity contrast of
$10^{-6}$, are far larger than the maximum curvature measured by Cohen
\& Nagel for two fluid layers with a viscosity contrast of
$10^{-3}$. The origin of these different outcomes is, at present, not understood. 

{\it Viscous withdrawal in 3D}\\
Recently, motivated by the thin stable spout created in the viscous
entrainment regime, Zhang analyzed the transition in the reverse direction, 
from viscous entrainment to selective withdrawal. The analysis focuses on the
regime where the viscosity of the fluid entrained is far smaller than
the viscosity of the entraining liquid, 
and constrains the spout shape to be nearly cylindrical
throughout~(\cite{Zhang04}). These 
simplifications allow the steady-state spout shape to be described
via a long-wavelength model. Surprisingly, results for the model show that, 
changing the boundary conditions on the interface, without changing
the material parameters, can profoundly change the nature of the shape
transition.  For some boundary conditions, the steady-state interface
deforms continuously with withdrawal flux 
from a spout to a hump across the transition. For other boundary
conditions, the steady-state interface changes discontinuously at the
transition. Thus, there appears to be a subtle interplay between the entraining 
flow and surface tension effects. As a result, the transition is 
strongly influenced by constraints on the large-scale shape of the
interface. 

{\it Emulsification}\\
Another extensively studied shape transition that has strong points of 
similarity with the selective withdrawal to viscous
entrainment transition occurs when a single liquid drop is emulsified
into several drops by an axisymmetric straining 
flow~(\cite{Taylor34,RallisonAcrivos78,Grace82,Stone94}). In both situations, 
an imposed flow
far from the interface induces flows near the interface between two
viscous liquids. The steady-state interface is deformed at low
flow rates and ``broken'' at high flow rates. The crucial differences
are that, for drop emulsification, 
there is no steady-state interface above the threshold flow rate. The
drop is simply stretched out indefinitely by the flow. Also, even in
the analog of the selective withdrawal regime, when
a steady-state shape exists for the drop, the flow dynamics are
different because the flow inside the drop must assume a form
satisfying global volume conservation. In contrast, for the two-layer
withdrawal experiment, the layer depth is always much larger than the
hump height. It is then reasonable to expect that the global volume
constraint does not introduce a significant modification to the flow 
dynamics. We will show this expectation is indeed borne out by results 
from the numerics. 

The viscosity contrast between the drop
and surrounding fluid strongly affects the 
deformation-to-burst transition. When the drop
is far less viscous than the surrounding liquid, the steady-state
shape approaches a cusp shape as the burst transition is approached
from below. In particular, the radius of curvature at the two,
elongated ends of the liquid drop is cut-off
on an exponentially small
lengthscale~(\cite{AcrivosLo78}). Long-wavelength analyses of 
the extended drop shape in this regime also show that the burst
transition corresponds to a saddle-node bifurcation in the
leading-order solution for the overall
drop shape~(\cite{Taylor64,Buckmaster73}). When the drop
viscosity is comparable with the surrounding liquid, the steady-state
shape remains nearly spherical as the burst transition is
approached. Recently, numerics and phenomenological arguments have shown
that the shape transition when the drop viscosity is equal to the
surrounding liquid viscosity corresponds to a saddle-node 
bifurcation~(\cite{Navot99,BlawCrisLoew02}). 

{\it Inviscid selective withdrawal}\\
Finally, we note that a similar flow-driven topological transition
exists at high Reynolds number when 
water drains out of a filled bathtub~(\cite{sautreaux01,lubin67}). In practice,
this is always accompanied by the formation of a vortex. 
More generally, withdrawal from two stratified layers
of inviscid fluids is relevant for transport in water storage
reservoirs, where often a layer of fresh water overlies a layer of
salty water~(\cite{imberger82}). Intriguingly, 
some of the results for the idealized problem of withdrawal from two
layers of perfectly inviscid fluids~(\cite{tuck84,vanden87,miloh93})
suggest that, 
for the inviscid fluid system, the transition from selective
withdrawal to full entrainment corresponds to the formation of a
singular shape on the steady-state interface. This has motivated many recent
theoretical and numerical studies, despite the fundamental 
difficulty that, without the
small-scale smoothing provided by viscosity and/or surface tension in
real life, the idealized problem is fundamentally ill-posed and can
only be approached via careful limiting processes. For the same
reason, direct comparison with experiments has also been
difficult. For our study, 
the most relevant and suggestive results deal with the role 
of the spatial dimension. Two-dimensional withdrawal 
differs significantly from axisymmetric
withdrawal~(\cite{forbes04,stokes05}). Also, in both 2D and
axisymmetric withdrawal, whether selective withdrawal or full
entrainment is realized can depend crucially on the transient evolution of
the interface~(\cite{hocking01}).

Our brief summary shows that studies of viscous flow driven
topological transitions have produced a wealth of surprises. The wide
range of behaviors observed indicate that seemingly subtle differences 
in the exact experimental configurations can have a dramatic effect
on the transition structure. Consequently, in order to make progress 
on the 3-D selective withdrawal problem, it is likely that experiments, 
simulations and theoretical calculations, all of which address the same 
flow geometry, will be needed. This is one reason why our study focuses on 
devising and analyzing a model withdrawal process that can be
directly compared with previous experiments~(\cite{CohenNagel02}).


==> model2.tex <==
%auto-ignore
% August 17 2006
%\section{Modeling selective withdrawal}
While features such as the absolute size of the hump or the detailed
hump shape depend on the precise geometry of the imposed withdrawal
flow and the boundary conditions, some features of the interface
evolution are expected to be robust. For example, the evolution of the 
interface, in particular how the hump height and curvature vary as 
$\tilde{Q}$ approaches $\tilde{Q}_c$, should be largely insensitive to 
these details. Even a simple model of selective
withdrawal would be able to reproduce these robust features and
therefore make contact between theory and experiment. Moreover, 
computing the solutions for a process which reproduces the experiment, 
with all of its physical effects and boundary conditions, is expensive, 
and therefore unlikely to yield the large dynamic range necessary to 
clearly display the fundamental nature of the transition. A highly 
idealized model, on the other hand, would fail to give results that 
can be compared in a meaningful way with the measurements. We therefore 
look to the experiments for guidance as to the ingredients necessary 
for a model to capture the essence of the flows associated with the
transition. 

In the experiment, there are two imposed 
lengthscales which are comparable with the observed
millimeter-sized hump height: $S_p$, the height  
of the tube, which ranges from $0.255 $ cm to $0.830$ cm, and the capillary
lengthscale $\ell_\gamma$, which is about $0.3$ cm and 
characterizes the relative importance
of surface tension and hydrostatic pressure. Deformations on 
lengthscales below $\ell_\gamma \equiv \sqrt{\gamma/\Delta \rho g}$ are
stabilized by surface tension. Deformations on lengthscales above
$\ell_\gamma$ are stabilized by hydrostatic pressure. All these
lengthscales are much smaller than the dimensions of the liquid layer 
which is $12$ cm deep and $30$ cm in extent. As will be shown in
greater detail in the next subsection, this difference in lengthscale
allows the experimental system to be well approximated by a simple
model, where liquid is withdrawn from two infinitely deep and
infinitely extended layers. Another 
simplification found in the experiments is that 
provided the tube height is sufficiently large, the interface 
deformation changes very little when the tube diameter is changed. 
This allows for modeling the withdrawal tube as a point sink.  

Since the tube height $S_p$ and the capillary lengthscale
$\ell_\gamma$ are comparable, both lengthscales are expected to influence
the dynamics. As a result, there are several reasonable ways to define
the Reynolds number, and 
it is unclear how the Reynolds number of the
withdrawal flow should change with
$S_p$ or $\ell_\gamma$. To avoid this ambiguity, 
we use the observed hump
height $\tilde{h}$ as the characteristic lengthscale and define the Reynolds
number $Re$ as 
$\rho \tilde{Q} \tilde{h} / (\mu 4 \pi S^2_p)$, where $\rho$ is the
density of the upper liquid, $\mu$ the viscosity of the upper
layer, and $\tilde{Q}/4 \pi S^2_p$ a typical flow rate. 
An estimate using parameters from the experiment 
yields $Re \approx 0.1$, indicating that inertial effects are small. 
The stress balance on the interface is therefore characterized by 
the capillary number, 
\beq
Ca = \frac{\mu}{\gamma}\frac{\tilde{Q}}{4 \pi S^2_p}
\eeq
a ratio of the strength of the viscous stresses exerted
by the flow relative to the Laplace pressure due to surface
tension. For a typical experiment, 
the transition from selective withdrawal to viscous
entrainment corresponds to a threshold capillary number $Ca_c$ in the range of
$10^{-3}$. Thus surface tension effects are strong even at the transition. 
%large variation in experimental measurement 
%only when you nondimensionalize by the capillary lengthscale

\subsection{Minimal Model}

Our derivation of a simple model withdrawal process begins by
considering the following idealized situation, depicted in
figure~\ref{fig:reservoir_bc}. A cylindrical tube of radius $R$ is
immersed in a large bath  
of viscous liquid. It is filled with a second, immiscible liquid. 
An axisymmetric withdrawal flow imposed in the
exterior fluid deforms the interface $S_I$ spanning the circular
opening with radius $a$ and creates a flow inside
the cylindrical tube of radius $R$. 
We use a cylindrical coordinate system where
$z=0$ corresponds to the tube opening, and $r=0$ coincides with the
tube centerline. 
For simplicity, we divide the interface into two parts. Near the
origin, for $0 \leq r \leq a$, the interface is deformed by the
withdrawal flow. At $r=a$, the interface $S_I$ is pinned. 
In other words, if $h(r)$ corresponds to the 
the interface shape and $z=0$ the interface shape with zero imposed flow, then
$h(r \geq a)=0$ for all flow rates. (To accomodate this pinning condition, 
we allow the contact angle of the interface at $r=a$ is allowed to
vary as a function of the flow rate. ) For $r > a$, the interface is
held to be perfectly flat. The Laplace pressure due to surface tension
effects, therefore, is nonzero only for $r \leq a$ and vanishes
outside that region.  This approximation is an inexpensive, but crude
way to include the effect of stratification between the two liquid
layers. In the experiment, the interface is essentially flat on radial
lengthscales beyond the capillary lengthscale $\ell_\gamma$. Very
approximately, therefore, the interface in the experiment deforms as
if it were confined within a cylindrical tube of radius
$\ell_\gamma$. We will see in section 4.2 that 
simulations performed which explicitly include the
stratification effect, and therefore involve a more extended
interface, give essentially the same results as the crude model used
here. 

Also for simplicity, the flow
dynamics in both liquids are assumed to be dominated by viscous
stresse and the two liquids are assumed to have identical
viscosities. The flows in the two liquids therefore satisfy Stokes
equation
\begin{equation}
  \mb{\nabla} \cdot \bfb{\sigma}= -\mb{\nabla}p + \mu \mb{\nabla}^2
\mb{u}= \mb{0}, 
  \quad \mb{\nabla}\cdot \mb{u} = \mb{0}
\end{equation}
where $\mb{u}$ is the velocity field, $p$ is the pressure and
$\bfb{\sigma}$ is the stress field.  Again, for simplicity, the
withdrawal in the model is driven by a point sink of strength
$\tilde{Q}$ located at a height $\tilde{S}$ above the interface in the
exterior. This corresponds to a withdrawal flow 
\beq
\mb{u}_\textrm{ext}(\mb{x}) = \frac{\tilde{Q}}{4 \pi | \mb{x}_S-\mb{x} |^3}
(\mb{x}_S-\mb{x})
\label{sink}
\eeq
where $\mb{x}_s = \tilde{S} \mb{e_z}$. This choice 
allows $\tilde{S}$ to be the only lengthscale imposed
by the flow, consistent with the experimental observation that hump
shape depends primarily on the height of the withdrawal tube and not
on its diameter. 

Since the flow dynamics in both layers are completely viscous, and
therefore described by linear equations, we can 
represent the velocity field as an integral over a
suitably defined closed
surface~(\cite{Lorentz07,Ladyzhenskaya63,pozirikidis92}). For example,
defining the closed interface as $S_I$ together with an interface
$S_\infty$ corresponding to a spherical shell centered at the origin 
with radius $R_\infty \rightarrow \infty$ and enclosing the liquid
in the upper layer, the velocity at a point ${\bf x}$ 
on the interface $S_I$ is given by
\beq
\frac{1}{2} \mb{u}(\mb{x}) =  - \int_{S_I} \bfb{J} \cdot 
  [ \mb{n} \cdot \bfb{\sigma} ] \, \rd S_{\mb{y}}
  - \int_{S_R} \mb{n} \cdot \bfb{K} \cdot \mb{u} \,\rd S_{\mb{y}} 
\label{basic_bint}
\eeq
where $\mb{y}$ is the point on the surface that you are integrating
over. Note we have also defined the 
surface normal $\mb{n}$ here to point into the closed region, hence
the negative signs in front of the surface integrals. 
The tensors $\mb{J}$ and $\mb{K}$ 
\begin{eqnarray}
  \mb{J}(\mb{r}) & = & \frac{1}{8\pi\mu} \left( \frac{\mb{1}}{r} +
\frac{\mb{rr}}{r^3} \right) \\
  \mb{K}(\mb{r}) & = & -\frac{3}{4\pi} \frac{\mb{rrr}}{r^5}
  \nonumber
\end{eqnarray}
and $\mb{r} = \mb{x}-\mb{y}$. 
Equation (\ref{basic_bint}) says that the velocity on
the interface is given by two surface integrals over $S_I$, one
summing over the normal stress exerted by fluid motion on $S_I$
(J-integral) and the second summing over the velocity on the interface
(K-integral). Similarly, 
the velocity ${\bf u}({\bf x})$ at a point ${\bf x}$ in the interior
of the upper layer is given by
\beq
\mb{u}(\mb{x}) =  - \int_{S_I} \bfb{J} \cdot 
  [ \mb{n} \cdot \bfb{\sigma} ] \, \rd S_{\mb{y}}
  - \int_{S_R} \mb{n} \cdot \bfb{K} \cdot \mb{u} \,\rd S_{\mb{y}} 
\label{upper_bint}
\eeq
while a point ${\bf x}$ in the lower layer lies outside the enclosed volume,
and therefore 
\beq
\mb{0} = - \int_{S_I} \bfb{J} \cdot 
  [ \mb{n} \cdot \bfb{\sigma}] \, \rd S_{\mb{y}}
  - \int_{S_R} \mb{n} \cdot \bfb{K} \cdot \mb{u} \,\rd S_{\mb{y}} 
\label{outside_upper_bint}
\eeq
For our purpose, the important point is that equation
(\ref{basic_bint}) provides an evolution equation for the interface,
provided we can find the normal stress distribution $\mb{n} \cdot
\bfb{\sigma}]$ on $S_I$. 

To do so, we need to find a physically reasonable 
way of approximating the flow induced inside the cydrical tube. 
The tube has radius $R$ and depth $H$. 
Both $R$ and $H$ are much larger than $\tilde{h}$, the hump height,
and the tube opening $a$. 
For simplicity, assume that $H$ is much larger than $R$ so that the
radial size is the only relevant lengthscale. 
The velocity field within the lower layer, or the liquid inside the
tube, then 
divides into three regions, as illustrated in figure~\ref{fig:reservoir_bc}. 
In region I, the velocity field is strongly affected by
the hump shape and the axial velocity $u_z$ is comparable 
with the radial velocity $u_r$. In region II, there
is a significant radial flow bringing liquid into and out of the hump
region. The strength of this 
radial flow decays as we move downwards away from
the interface and below a distance $h_2$ becomes negligible. Liquid in
region III, therefore, is essentially stagnant, with the pressure
distribution being spatially uniform and constant over time. Since 
we have chosen the pressure in the upper 
layer to be zero far from the interface, the pressure in region
III of the lower layer need not equal to this reference pressure and 
will in general has the value $p_0$. 
\begin{figure}
  \centering
  \includegraphics[width=0.65\textwidth]{figures/reservoir_bc.eps}
  \caption{Schematic of the large reservoir set-up used in deriving
  the appropriate boundary condition across the surface $S_R$. The
  hump height $\tilde{h}$ and lateral extent $a$ are much smaller than
  the container radius $R$. The container radius $R$ is smaller than
  its depth $H$. }
  \label{fig:reservoir_bc}
\noindent\rule{5.3in}{.5mm}
\end{figure}

We can estimate $h_2$, the vertical extent
of region II, by first considering the tangential stress continuity
across $S_R$. For a strongly deformed hump, the tangential
stress exerted on $S_R$ by the flow in region I is roughly $\mu
(u_z/{a})$. Balancing it
against the tangential stress due to the radial flow in region II
at $S_R$ yields
\beq
\mu \frac{u_z}{a} \sim \mu \frac{u_r}{h_2} 
\eeq
which in turn implies
\beq
\frac{u_r}{u_z}
\sim \frac{h_2}{{a}}
\label{tangscale}
\eeq 
Next we balance $u_z (\pi {a}^2)$, 
the volume flux out of $S_R$ at the bottom of the hump, against $u_r (2 \pi R
h_2)$, the volume flux of fluid into the hump from the edge of the
container. This yields 
\beq
\frac{u_r}{u_z} \sim \frac{\pi {a}^2}{2 \pi R h_2} \ .
\label{fluxscale}
\eeq
Scaling relations (\ref{tangscale}) and (\ref{fluxscale}) together
shows $h_2$ depends on ${a}$ and the container size as 
\beq
\frac{h_2}{{a}} \sim \sqrt{ \frac{{a}}{R} }\ .
\label{h2scale}
\eeq

We can approach a scenario which roughly approximates 
the experimental situation of two liquid layers
overlying each other by considering the limit where 
the tube radius $R$ is made larger and larger while the tube
opening $a$ remains fixed. As this limit proceeds, the vertical extent
of region II becomes smaller and smaller relative to
$a$. In the limit ${a}/R \rightarrow 0$, region II simply
shrinks into a surface of zero thickness, here denoted by $S_R$. At 
$S_R$ are that the stress distribution in region I merges continuously
with the stress distribution in region III. Since the flow is stagnant
in region III, the tangential stress at $S_R$ is $0$ and the normal
stress distribution simply corresponds to a uniform pressure
distribution $p_0$.  

We are now ready to derive an evolution equation for the interface. 
To begin, we note that, $S_R$ and $S_I$ together comprise a closed
surface, enclosing liquid in region I. Therefore, using the boundary
integral formulation, the velocity of a point $\mb{x}$ 
on the combined closed surface $S_R + S_I$, defined with outward
pointing normal, is given by
\begin{eqnarray}
 \frac{1}{2} \mb{u}(\mb{x}) & = &  \int_{S_I} \bfb{J} \cdot 
  [ \mb{n} \cdot \bfb{\sigma} ] \, \rd S_{\mb{y}}
  + \int_{S_I} \mb{n} \cdot \bfb{K} \cdot \mb{u} \,\rd S_{\mb{y}} \\
  & & + \int_{S_R} \bfb{J} \cdot 
  [ \mb{n} \cdot \bfb{\sigma} ] \, \rd S_{\mb{y}}
  + \int_{S_R} \mb{n} \cdot \bfb{K} \cdot \mb{u} \,\rd S_{\mb{y}}
  \nonumber 
\label{comb_bint}
\end{eqnarray}
We already know that, at the reservoir surface $S_R$, the normal
stress distribution is simply $p_0 \mb{n}$. To obtain the velocity on
the fluid interface $S_I$, we simply 
adding (\ref{basic_bint}) and (\ref{comb_bint}) together for $\mb{x}$
on $S_I$. The K-integral over $S_I$ cancel, reflecting the tangential
stress condition which causes
the tangential velocity gradient across an interface separating two
liquids of equal viscosity is continuous. The J-integral over
$S_I$ now involves the jump of the normal stress across $S_I$, instead
of the normal stress distribution itself. 
We thus obtain
\begin{eqnarray}
  \frac{1}{2} \mb{u}(\mb{x}) & = & \int_{S_I} \bfb{J} \cdot 
 [ \mb{n} \cdot \bfb{\sigma} ]_{-}^{+}\, \rd S_{\mb{y}} \\
  & & + \int_{S_R} \bfb{J} \cdot \mb{n} \ p_0 \, \rd S_{\mb{y}}
  + \int_{S_R} \mb{n} \cdot \bfb{K} \cdot \mb{u} \,\rd S_{\mb{y}} \nonumber
\end{eqnarray}
where the jump in the normal stress distribution 
$[ \mb{n} \cdot \bfb{\sigma} ]_{-}^{+}$ is, from the normal stress
boundary condition, simply the Laplace pressure
$\gamma 2 \tilde{\kappa} \mb{n}$ where $\kappa$ is the mean surface
curvature. We thus arrive at an integral evolution equation for the
liquid interface $S_I$, provided the velocity field on the reservoir
surface $S_R$ is known
\begin{eqnarray}
\label{usI}
  \mb{u}(\mb{x}) & = & \int_{S_I} \bfb{J} \cdot 
  \mb{n} \left[ \gamma 2 \tilde{\kappa} \right]\, \rd S_{\mb{y}}\\
  & & + \int_{S_R} \bfb{J} \cdot \mb{n} \ p_0 \, \rd S_{\mb{y}}
  + \int_{S_R} \mb{n} \cdot \bfb{K} \cdot \mb{u} \,\rd S_{\mb{y}} \nonumber\\
  & & + \ \mb{u}_\textrm{ext}\left(\mb{x}\right) 
\nonumber
\end{eqnarray}
The last term corresponds to the sink flow~(\ref{sink}) imposed in the
upper layer.  The velocity on $S_R$, 
which is needed to evaluate (\ref{usI}), can be obtained by adding
(\ref{outside_upper_bint}) and (\ref{comb_bint}) for a point $\mb{x}$
on the reservoir surface $S_R$. 
\begin{eqnarray}
\label{usII}
  \frac{1}{2} \mb{u}(\mb{x}) & = & \int_{S_I} \mb{J} \cdot 
  \mb{n} \left[ \gamma 2 \tilde{\kappa} \right]\, \rd S_{\mb{y}} \\
  & & + \int_{S_R} \mb{J} \cdot \mb{n} \ p_0 \, \rd S_{\mb{y}} 
  + \int_{S_R} \mb{n} \cdot \mb{K} \cdot \mb{u} \,\rd S_{\mb{y}} 
\nonumber
\end{eqnarray}
Since $S_R$ lies outside the closed interface $S_I + S_\infty$ defined for
(\ref{outside_upper_bint}), the integral contribution to points on
$S_R$ sums up to $0$. Solving (\ref{usI}) and (\ref{usII})
simultaneously yields the 
velocity on the interface. To obtain the steady-state interface shape,
we update the interface using the kinematic boundary condition, 
\begin{equation}
  \label{eq:kinematic_bc}
  \frac{d\mb{x}}{dt} = \mb{u}(\mb{x}) \textrm{ for } \mb{x} \in S_I \
  . 
\end{equation}
We then solve
(\ref{usI}) and (\ref{usII}) using the updated interface. The
procedure is repeated until either a steady-state is obtained or the
interface is drawn into the sink. 

Figure~\ref{fig:surface_185.49_clean} illustrates the final,
simplified model of viscous withdrawal from two liquid layers. 
We will show in section 4 that the interface evolution obtained using 
these conditions agrees well with that measured in the experiments as 
well as more expensive numerical results obtained using a closed surface 
which encloses all the liquid in the lower layer.
\begin{figure}
  \centering
  \includegraphics[width=0.7\textwidth]{figures/surface_185.49_clean.eps}
  \caption{Simplified numerical model of selective withdrawal. The
  closed surface in the boundary integral formulation is comprised of
  the liquid interface $S_I$ and a fictious surface $S_R$ representing
  reservoir condition. Across $S_R$, the fluid pressure jumps by an amount
  $P_0$. }
  \label{fig:surface_185.49_clean}
\noindent\rule{5.3in}{.5mm}
\end{figure}

Finally we nondimensionalize the withdrawal problem
via the following characteristic length-, velocity- and stress-scales
\beq
\hat{\ell} = a \qquad \hat{u} = \frac{\gamma}{\mu} 
\qquad \hat{p} = \frac{\gamma}{a} 
\label{nondim}
\eeq
The dimensionless withdrawal flux is then 
\begin{displaymath}
  Q = \frac{\mu \tilde{Q}/a^2}{\gamma}
\end{displaymath}
and is equivalent to a capillary number $Ca$. 

